Game Theory on the Ground: The Effect of Increased Patrols on Deterring Poachers

Applications of artificial intelligence for wildlife protection have focused on learning models of poacher behavior based on historical patterns. However, poachers' behaviors are described not only by their historical preferences, but also their reaction to ranger patrols. Past work applying machine learning and game theory to combat poaching have hypothesized that ranger patrols deter poachers, but have been unable to find evidence to identify how or even if deterrence occurs. Here for the first time, we demonstrate a measurable deterrence effect on real-world poaching data. We show that increased patrols in one region deter poaching in the next timestep, but poachers then move to neighboring regions. Our findings offer guidance on how adversaries should be modeled in realistic game-theoretic settings.

==> figures/bar_stats.tex <==
\begin{tikzpicture}
\pgfplotsset{
  %scale only axis,
  width=.5\linewidth,
  height=.36\linewidth,
  xtick pos=left,
  ytick pos=left,
  tick label style={font=\tiny},
%   label style={font=\tiny},
  ymajorgrids=true,
  ybar,
  xticklabel style={/pgf/number format/1000 sep=}, % display as 2000 instead of 2,000
}


\begin{axis}[ 
  at={(0, .35\linewidth)},
  bar width=2pt,
%   xlabel={(a)},
%   title={\textsc{Synthetic Data}},
%   ylabel style={align=center}, 
%   ylabel absolute, ylabel style={xshift=-1.8cm, yshift=-.4cm},
  title={\small{(a) Patrol effort (km)}},
%  ylabel={\footnotesize{Reward}},
  xlabel near ticks,
  ylabel near ticks,
%  legend style={
%    align=left,
%    at={(1,1.8)},
%    legend columns=1,
%    row sep=0cm,
%    font=\scriptsize, 
%    draw=none,
%    fill=none,},
%   ymin=0,
%   ymax=.8,
%  xmin=0,
%  xmax=500,
]
\addplot[blue,fill] table[x=year,y=effort_km, col sep=comma]{data/stats.csv};
\end{axis}

\begin{axis}[ 
  at={(.5\linewidth, .35\linewidth)},
  bar width=2pt,
  title={\small{(b) Average effort (km/visit)}},
  xlabel absolute, xlabel style={xshift=0, yshift=-1},
%  xlabel={\footnotesize{Year}},
%   title={\textsc{Synthetic Data}},
%   ylabel style={align=center}, 
%   ylabel absolute, ylabel style={xshift=-1.8cm, yshift=-.4cm},
%   ylabel={\scriptsize{Performance}},
%   xlabel near ticks,
%   ylabel near ticks,
  legend style={
    align=left,
    at={(1.2,1.55)},
    legend columns=1,
    font=\scriptsize, 
    draw=none,
    fill=none,},
    ymin=0,
%   ymax=.8,
%  xmin=0,
%  xmax=500,
]
\addplot[blue,fill] table[x=year,y=avg_effort, col sep=comma]{data/stats.csv};
\end{axis}

\begin{axis}[ 
  bar width=2pt,
  at={(0\linewidth, 0\linewidth)},
%   xlabel={\footnotesize{(c)}},
%   title={\textsc{Synthetic Data}},
%   ylabel style={align=center}, 
%   ylabel absolute, ylabel style={xshift=-1.8cm, yshift=-.4cm},
%   ylabel={\scriptsize{Performance}},
  title={\small{(c) Illegal activity}},
  xlabel near ticks,
%   ylabel near ticks,
%  ytick={.5, .6},
  legend style={
    align=left,
    at={(1.2,1.55)},
    legend columns=2,
    font=\scriptsize, 
    draw=none,
    fill=none,},
%   ymin=0,
%   ymax=.8,
%  xmin=-4,
%  xmax=45,
]
\addplot[red,fill] table[x=year,y=illegal_activity, col sep=comma]{data/stats.csv};
\end{axis}

\begin{axis}[ 
  bar width=2pt,
  at={(.5\linewidth, 0\linewidth)},
%   xlabel={\footnotesize{(c)}},
%   title={\textsc{Synthetic Data}},
%   ylabel style={align=center}, 
%   ylabel absolute, ylabel style={xshift=-1.8cm, yshift=-.4cm},
%   ylabel={\scriptsize{Performance}},
  title={\small{(d) CPUE}},
  xlabel near ticks,
  %%%%%%%%%%%%
  % prevent .08 from showing up as 8 * 10^-2
  yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=2
  },
  scaled y ticks=false, 
  %%%%%%%%%%%%
%   ylabel near ticks,
%  ytick={.5, .6},
  legend style={
    align=left,
    at={(1.2,1.55)},
    legend columns=2,
    font=\scriptsize, 
    draw=none,
    fill=none,},
   ymin=0,
%   ymax=.8,
%  xmin=-4,
%  xmax=45,
]
\addplot[red,fill] table[x=year,y=CPUE, col sep=comma]{data/stats.csv};
\end{axis}

%\node[anchor=north] (a1) at (.11\linewidth, -.25){\scriptsize{(a)}};
%\node[anchor=north] (a1) at (.42\linewidth, -.25){\scriptsize{(b)}};
%\node[anchor=north] (a1) at (.73\linewidth, -.25){\scriptsize{(c)}};

% used to show overall space
% \draw (current bounding box.south east) rectangle (current bounding box.north west);

% \begin{axis}[
%            ybar,
%%            symbolic x coords={0--2,2--5,5--10,10--20,20--50,50+},
%%            symbolic x coords={2010,,,,2014,,,,2018,,},
%            %xtick=data,
%            xlabel={\footnotesize{Year}},
%            ylabel={\footnotesize{Average effort (km)}},
%        ]
%        \addplot table[x=year,y=effort_km, col sep=comma]{data/stats.csv};
%%        \addplot [green, thin, mark=none] table [x=year, y=monotone, col sep=comma] {data/reward_vary_monotonicity.csv};
%    \end{axis}
\end{tikzpicture}
